"Public(s)-in-the-Loop": Facilitating Deliberation of Algorithmic Decisions in Contentious Public Policy Domains

This position paper offers a framework to think about how to better involve human influence in algorithmic decision-making of contentious public policy issues. Drawing from insights in communication literature, we introduce a "public(s)-in-the-loop" approach and enumerates three features that are central to this approach: publics as plural political entities, collective decision-making through deliberation, and the construction of publics. It explores how these features might advance our understanding of stakeholder participation in AI design in contentious public policy domains such as recidivism prediction. Finally, it sketches out part of a research agenda for the HCI community to support this work.

==> misc.tex <==
This framework is based on theories of deliberative democracy and is intended to expand the existing conceptual toolkit by introducing a ``public(s)-in-the-loop'' approach. Using the vocabulary of political philosophy and communication theory, we enumerate three features that are central to this approach: reasonable pluralism, collective decision-making through deliberation, and the construction of publics. We then explore how these features might advance our understanding of human influence over algorithmic decision-making in highly contentious public policy domains such as recidivism prediction. Finally, we sketch out part of a research agenda for the HCI community to support this work.

a situation when an algorithmic decision has to be made about a public policy issue and where there is pervasive reasonable disagreement but no universally applicable normative standard -- or ``ground truth'' -- to settle such disagreement. 

This framework takes seriously the contentious nature of many public policy issues because in a liberal democratic society citizens can reasonably disagree with each other on the ``right'' answers. It does not try to offer the ``right'' answer by simply aggregating different individual preferences but rather argues that through public deliberation and social learning, a more acceptable answer might emerge from collective decision making. 

It therefore shifts the questions of fairness to the processes and procedures for determining which social values to be considered in designing algorithmic decision making systems. 

Scholars in communications have long argued that creating a ``public sphere'' to invite more citizens into the deliberation and debate on high-stake public decision-making is of vital importance for modern democracies \cite{habermas1991structural,calhoun1992habermas}. Previous work in HCI \cite{disalvo2009design,DiSalvo:2012:AD:2341007} also emphasizes the importance of forming and constructing the publics around high-stake social issues through design. Wider public participation in the debates on algorithmic decision-making, on the one hand, could tip the balance toward things working in the public interest and inform better policy-making. On the other hand, it will also expose the often invisible tensions, conflicts and politics encoded in these seemingly neutral algorithms and raise better public awareness. 


Literature on publics adds three basic concerns to our conceptual toolkit: 

Methods for stakeholder participation in AI design


\section{Using the Framework for Analysis}
These three features -- publics as plural political entities, collective decision-making through deliberation, and the construction of publics -- are central themes in the discussion of publics and democracy. They have so far been relatively overlooked in the debates on the governance of algorithmic decision making systems. To illustrate this idea, think of the cases that have captivated the public discussion on the fairness of the recidivism prediction algorithms.

These three concerns -- collective decision making, the importance of deliberation and the construction of publics -- are central themes in the discussion of publics and democracy. They have so far been largely overlooked in the debates on the governance of algorithmic decision making systems. To illustrate this idea, think of the cases that have captivated the public discussion on the fairness of the recidivism prediction algorithms. 

A major problem with such discussion and other similar dilemmas is that they look at these choices as if they were exclusively mathematical problems even though they raise a distinctively political question. Recidivism prediction cases ask: Which fairness metrics are most appropriate in a given context?  

Instead, 

This point generalizes to other algorithmic decision-making systems. 

How such political concerns are taken into considerations when we design future human-centered AI systems is a question rife for interdisciplinary cooperation.  

Dewey \cite{dewey1927public} highlighted the importance of public deliberation in political decision making as well as the role of progressive education (e.g., the press) to forge a democratic public.

``exchange of the reasons'' -- aggregation of individual preference is not suffice as only through the exchange of reasons, different members of publics will learn more deeply about the problems and learn from those who are adversely affected by algorithimic decision making.

Instead of solely focusing on improving structures and mechanisms that enable governing, we should also consider through our projects to create spaces for revealing and confronting power relations. 

creating and enabling these spaces of contest. 

\begin{figure}
  \lefting
  \includegraphics[width=230]{figures/framework.fairness.jpeg}
  \caption{A ``Public(s)-in-the-Loop'' Approach introduces three basic concerns to our conceptual tookit: Collective decision making, the importance of deliberation, and the construction of publics.}
  \label{framework}
\end{figure}

\begin{figure}
\centering
  \includegraphics[width=220]{figures/framework.001.jpeg}
  \caption{A ``Public(s)-in-the-Loop'' approach introduces three features to our conceptual tookit: publics as plural political entities, collective decision-making through deliberation, and the construction of publics.}
    \vspace*{-0.1in}
  \label{framework}
\end{figure}

\jason{Figure 1 feels 'sparse'. It doesn't feel like a great use of space right now, because the information density feels low. Maybe contrast it with other points in the possible design space?}
